PRIMO: Private Regression in Multiple Outcomes

We introduce a new private regression setting we call Private Regression in Multiple Outcomes (PRIMO), inspired by the common situation where a data analyst wants to perform a set of $l$ regressions while preserving privacy, where the features $X$ are shared across all $l$ regressions, and each regression $i \in [l]$ has a different vector of outcomes $y_i$. Naively applying existing private linear regression techniques $l$ times leads to a $\sqrt{l}$ multiplicative increase in error over the standard linear regression setting. We apply a variety of techniques including sufficient statistics perturbation (SSP) and geometric projection-based methods to develop scalable algorithms that outperform this baseline across a range of parameter regimes. In particular, we obtain no dependence on l in the asymptotic error when $l$ is sufficiently large. Empirically, on the task of genomic risk prediction with multiple phenotypes we find that even for values of $l$ far smaller than the theory would predict, our projection-based method improves the accuracy relative to the variant that doesn't use the projection.

==> text/discussion.tex <==
\section{discussion}

\begin{itemize}
    \item Open problem - in regression setting $1$ can we obtain non-vacuous bounds and improved error tradeoff in the large Y regime? 
    
\end{itemize}

==> text/full_results.tex <==
\subsection{Table of Experimental Results}
\begin{table}[h]
\centering
  \caption{Summary of Results ($d=25$)}
  \label{tab:results}
  \begin{tabular}{ccccl}
    \toprule
    Dataset & $l$ & Method & $R^2$ & $Log(R)$ \\
    \midrule
    1K Genome & 1 & Private Gauss & .86 & 3.45 \\
     &  & Private Proj & -.73 & 6.0 \\
     & 11 & Private Gauss & .72 & 4.1 \\
     &  & Private Proj & .67 & 4.28 \\
     & 50 & Private Gauss & .21 & 5.16 \\
     &  & Private Proj & .69 & 4.27 \\
     & 101 & Private Gauss & -.73 & 5.91 \\
     &  & Private Proj & .69 & 4.29 \\
     & 201 & Private Gauss & -4.49 & 7.04 \\
     &  & Private Proj & .6 & 4.52 \\
     & 601 & Private Gauss & -10.66 & 7.83 \\
     &  & Private Proj & .56 & 4.65 \\
     & 1001 & Private Gauss & -17.69 & 8.31 \\
     &  & Private Proj & .59 & 4.61 \\
     & 2001 & Private Gauss & -45.4 & 9.21 \\
     &      & Private Proj & .56 & 4.67 \\
     & 5000 & Private Gauss & -120.7 & 10.18 \\
     &      & Private Proj & .54 & 4.7 \\
     & 10000 & Private Gauss & -301.8 & 11.1 \\
     &       & Private Proj & .39 & 5.0 \\
     & 25000 & Private Gauss & -701.3 & 11.94 \\
     &       & Private Proj & .39 & 4.98 \\
     & 50000 & Private Gauss & -1316.4 & 12.57 \\
     &       & Private Proj & .39 & 4.98 \\
     & 100000 & Private Gauss & -3122.3 & 13.43 \\
     &        & Private Proj & .12 & 5.34 \\
    dbGaP & 1 & Private Gauss & .99 & 2.95 \\
     & & Private Proj & -.14 & 7.42 \\
     & 11 & Private Gauss & .98 & 3.3 \\
     & & Private Proj & -.12 & 7.22 \\
     & 50 & Private Gauss & .92 & 4.46 \\
     & & Private Proj & .81 & 5.33 \\
     & 101 & Private Gauss & .81 & 5.26 \\
     & & Private Proj & .87 & 4.93 \\
     & 201 & Private Gauss & .74 & 5.55 \\
     & & Private Proj & .93 & 4.37 \\
     & 601 & Private Gauss & .002 & 6.89 \\
     & & Private Proj & .94 & 4.11 \\
     & 1001 & Private Gauss & -.83 & 7.50 \\
     & & Private Proj & .94 & 4.09 \\
     & 2001 & Private Gauss & -2.37 & 8.12 \\
     &      & Private Proj & .95 & 3.98 \\
     & 5000 & Private Gauss & -9.29 & 9.23 \\
     &      & Private Proj & .94 & 4.14 \\
     & 10000 & Private Gauss & -27.4 & 10.25 \\
     &       & Private Proj & .93 & 4.34 \\
     & 25000 & Private Gauss & -66.3 & 11.12 \\
     &       & Private Proj & .93 & 4.33 \\
     & 50000 & Private Gauss & -124.4 & 11.74 \\
     &       & Private Proj & .93 & 4.25 \\
     & 100000 & Private Gauss & -289.7 & 11.58 \\
     &        & Private Proj & .92 & 4.44 \\

    \bottomrule
  \end{tabular}
  \label{tbl}
\end{table}

% full table
% \begin{table}[h]
% \centering
%   \caption{Summary of Results ($d=25$)}
%   \label{tab:results}
%   \begin{tabular}{ccccl}
%     \toprule
%     Dataset & l & Method & $R^2$ & $Log(R)$ \\
%     \midrule
%     1K Genome & 1 & Private Gauss & .86 & 3.45 \\
%      &  & Private Proj & -.73 & 6.0 \\
%      & 11 & Private Gauss & .72 & 4.1 \\
%      &  & Private Proj & .67 & 4.28 \\
%      & 50 & Private Gauss & .21 & 5.16 \\
%      &  & Private Proj & .69 & 4.27 \\
%      & 101 & Private Gauss & -.73 & 5.91 \\
%      &  & Private Proj & .69 & 4.29 \\
%      & 201 & Private Gauss & -4.49 & 7.04 \\
%      &  & Private Proj & .6 & 4.52 \\
%      & 401 & Private Gauss & -7.07 & 7.46 \\
%      &  & Private Proj & .63 & 4.48 \\
%      & 601 & Private Gauss & -10.66 & 7.83 \\
%      &  & Private Proj & .56 & 4.65 \\
%      & 801 & Private Gauss & -18.57 & 8.36 \\
%      &  & Private Proj & .56 & 4.67 \\
%      & 1001 & Private Gauss & -17.69 & 8.31 \\
%      &  & Private Proj & .59 & 4.61 \\
%      & 1201 & Private Gauss & -18.9 & 8.36 \\
%      &  & Private Proj & .64 & 4.45 \\
%      & 1401 & Private Gauss & -28.6 & 8.77 \\
%      &      & Private Proj & .61 & 4.54 \\
%      & 1601 & Private Gauss & -42.88 & 9.16 \\
%      &      & Private Proj & .43 & 4.93 \\
%      & 1801 & Private Gauss & -35.6 & 8.98 \\
%      &      & Private Proj & .59 & 4.58 \\
%      & 2001 & Private Gauss & -45.4 & 9.21 \\
%      &      & Private Proj & .56 & 4.67 \\
%      & 5000 & Private Gauss & -120.7 & 10.18 \\
%      &      & Private Proj & .54 & 4.7 \\
%      & 10000 & Private Gauss & -301.8 & 11.1 \\
%      &       & Private Proj & .39 & 5.0 \\
%      & 25000 & Private Gauss & -701.3 & 11.94 \\
%      &       & Private Proj & .39 & 4.98 \\
%      & 50000 & Private Gauss & -1316.4 & 12.57 \\
%      &       & Private Proj & .39 & 4.98 \\
%      & 100000 & Private Gauss & -3122.3 & 13.43 \\
%      &        & Private Proj & .12 & 5.34 \\
%     dbGaP & 1 & Private Gauss & .99 & 2.95 \\
%      & & Private Proj & -.14 & 7.42 \\
%      & 11 & Private Gauss & .98 & 3.3 \\
%      & & Private Proj & -.12 & 7.22 \\
%      & 50 & Private Gauss & .92 & 4.46 \\
%      & & Private Proj & .81 & 5.33 \\
%      & 101 & Private Gauss & .81 & 5.26 \\
%      & & Private Proj & .87 & 4.93 \\
%      & 201 & Private Gauss & .74 & 5.55 \\
%      & & Private Proj & .93 & 4.37 \\
%      & 401 & Private Gauss & .31 & 6.54 \\
%      & & Private Proj & .94 & 4.22 \\
%      & 601 & Private Gauss & .002 & 6.89 \\
%      & & Private Proj & .94 & 4.11 \\
%      & 801 & Private Gauss & -.39 & 7.22 \\
%      & & Private Proj & .95 & 4.06 \\
%      & 1001 & Private Gauss & -.83 & 7.50 \\
%      & & Private Proj & .94 & 4.09 \\
%      & 1201 & Private Gauss & -1.22 & 7.7 \\
%      &  & Private Proj & .94 & 4.11 \\
%      & 1401 & Private Gauss & -1.76 & 7.91 \\
%      &      & Private Proj & .94 & 4.11 \\
%      & 1601 & Private Gauss & -2.35 & 8.11 \\
%      &      & Private Proj & .94 & 4.19 \\
%      & 1801 & Private Gauss & -2.11 & 8.04 \\
%      &      & Private Proj & .95 & 4.05 \\
%      & 2001 & Private Gauss & -2.37 & 8.12 \\
%      &      & Private Proj & .95 & 3.98 \\
%      & 5000 & Private Gauss & -9.29 & 9.23 \\
%      &      & Private Proj & .94 & 4.14 \\
%      & 10000 & Private Gauss & -27.4 & 10.25 \\
%      &       & Private Proj & .93 & 4.34 \\
%      & 25000 & Private Gauss & -66.3 & 11.12 \\
%      &       & Private Proj & .93 & 4.33 \\
%      & 50000 & Private Gauss & -124.4 & 11.74 \\
%      &       & Private Proj & .93 & 4.25 \\
%      & 100000 & Private Gauss & -289.7 & 11.58 \\
%      &        & Private Proj & .92 & 4.44 \\

%     \bottomrule
%   \end{tabular}
%   \label{tbl}
% \end{table}


==> text/related_work.tex <==
\section{Related Work}\label{sec:rel_work}

\input{text/rel_work_linreg}


%\cite{proj} bound the accuracy of their mechanism with respect to the \emph{expected} mean squared error. Due to the necessity of analyzing the error of private regression with a high probability bound, rather than expected error, we prove a high probability error bound for the accuracy of the projection mechanism (Theorem~\ref{thm:proj-acc}). This requires application of the Hanson-Wright Inequality for anisotropic sub-Gaussian variables \cite{vershynin}. 




